Causality and Batch Reinforcement Learning: Complementary Approaches To Planning In Unknown Domains

Reinforcement learning algorithms have had tremendous successes in online learning settings. However, these successes have relied on low-stakes interactions between the algorithmic agent and its environment. In many settings where RL could be of use, such as health care and autonomous driving, the mistakes made by most online RL algorithms during early training come with unacceptable costs. These settings require developing reinforcement learning algorithms that can operate in the so-called batch setting, where the algorithms must learn from set of data that is fixed, finite, and generated from some (possibly unknown) policy. Evaluating policies different from the one that collected the data is called off-policy evaluation, and naturally poses counter-factual questions. In this project we show how off-policy evaluation and the estimation of treatment effects in causal inference are two approaches to the same problem, and compare recent progress in these two areas.

==> OPPE_firstdraft.tex <==

\section{Off-Policy Policy Evaluation: Causal Approaches}\label{sec:OPPE}
As we have briefly discussed in the introduction, offline reinforcement learning rests on the same counterfactual thinking as causal inference does (counterfactual inference). With missing data or limited access to data, both of them deal try to extract some information from historical data or observations and apply it to counterfactual scenarios, where it is too costly to launch experiments and collect data or too controversial even unethical to launch online exploration (e.g. healthcare applications). In this section, we focus on causality based approaches in solving off-policy policy evaluation (OPPE) problem, which is the key challenge in off-line reinforcement learning and we shall show that OPPE can either be reformulated as a counterfactual inference problem in a model-free fashion or can be solved in a model-based manner where the model is constructed by counterfactual thinking.

In this section, we first give a quick review about Markov Decision Processes (MDP) \cite{Bel} and introduce the off-policy policy evaluation problem. We then give an overview of OPPE methods, including \testbf{model-free} and \testbf{model-based} methods, and show how causality can be used in each approach. Finally, we make a comparison between causality-based and existing methods for OPPE, where we illustrate the advantages of incorporating causality into OPPE.       

\subsection{An Overview of Offline Reinforcement Learning}
We begin our overview of offline reinforcement learning using the notational standard MDPNv1 \cite{thomas2015notation}. Generally, in a reinforcement learning problem, the task of the agent who are supposed to make decisions sequentially in a dynamic environment, is to find an optimal policy maximizing the expected long term return, based on rewards received at each time step. The challenge of reinforcement learning is that the agent does not have complete information about the dynamic environment and tries to identify high-reward behavior patterns by interacting with the unknown environment. This sequential decision-making process under some dynamic environment is modeled by Markov Decision Process \cite{sutton2018reinforcement}, denoted by a tuple $\MDP$, where
\begin{itemize}
	\item We use $\step$ to denotes the time step, where $\NZ$ denotes the natural numbers {\em including zero}.

  \item $\sset$ is the state space that the agent can be in, and is called the {\em state set}. We note that the state of the environment at time $t$ is a random variable denoted by $\st{t}$. We will typically use $s$ to denote an element of the state set.
  \item $\aset$ is the action space, i.e, the set of possible actions the agent can perform. The action at time $t$ is denoted by $\at{t}$, while $a$ denotes an element of the action set.
  \item $\rset$ is the set of possible rewards, defined as $\rsetdef$. Additionally, instantaneous reward at time $t$ is $r(s_t,a_t)$, where $s_t, a_t$, as defined above are the current state and action respectively. 
  \item $\Tdef$ is called the {\em transition function}. For all $(s,a,s',t) \in \sset \times \aset \times \sset \times \NZ$, let $\Tfun(s,a,s')\coloneqq\Pr(\st{t+1}=s' \mid \st{t}=s, \at{t}=a)$. In other words, $\Tfun$ characterizes the distribution over states at time $t+1$ given the state and action at time $t$. We note that this distribution is only conditional on the last state and action and is independent of the previous history, indicating that the sate transition is \textit{markovian}. 
   \item $\isset$ is the initial distribution of states defined as $\issetdef$ and $\D$ is the discount factor defined as $\Ddef$. 
\end{itemize}
As we mentioned above, the goal of the agent is to find a policy $\pdef$ defined as a probability distribution over $\sset\times\aset$, such that by following this policy, the agent maximize the expected return. 


Off-policy evaluation, or more broadly speaking, policy evaluation is about measuring the quality of a given policy, and this measurement rests on the sample trajectories either generated by the policy to be evaluated (on-policy) or by some different policy or policies (off-policy). We note that by quality of a policy, we mean the expected return when following this policy, i.e., $\mathbb{E}_{\tau\sim p}\{\sum_{i=0}^H r(s_t,a_t)\}$, where $\tau=\left(s_{0}, a_{0}, \dots, s_{H}\right)$ is the trajectory, a series of state-action pairs generated by the given policy, which follows a distribution $p$ closely related to the policy, as we shall detail later. 
Generally, off-policy policy evaluation is more challenging than on-policy policy evaluation, since there is a distributional mismatch between the policy we are interested in and the policy  
that is actually implemented in the MDP model for generating those sample trajectories. In the sequel, we refer to the interested policy as the target policy, denoted by $\pi$ while to the data-generating policy as the behavioral policy $\mu$. To see this mismatch, we only need to realize that sample trajectories are in fact a series of state-action pairs sampled from the trajectory distribution. For example, for a MDP model $M$, a given behavioral policy $\mu$, and a sample trajectory of $H + 1$ states and actions, $\tau=\left(s_{0}, a_{0}, \dots, s_{H}\right)$,  then the distribution of $\tau$ as $p_{M,\mu}=d_{0}\left(s_{0}\right) \prod_{t=0}^{H-1}\left[\Tfun(s_t,a_t,s_{t+1}) \mu\left(s_{t}, a_{t}\right)\right]$, where $d_0$, as introduced at the beginning of this section, is the initial state distribution. Obviously, for the target policy $\pi\neq\mu$, we have the mismatch $p_{M,\mu}\neq p_{M,\pi}$, meaning that this sample trajectory $\tau$ cannot be directly applied to estimating the expected return $\mathbb{E}_{\tau\sim p_{M,\pi}}\{\sum_{i=0}^H r(s_t,a_t)\}$.



Offline reinforcement learning aims at learning a new policy based on only historical observations and additional interactions with the unknown environment are not permitted \cite{lange2012batch}. The inability of receiving feedback from the environment avoids potential costs and safety issues but also poses a great challenge to the learning process. As observed in \cite{fujimoto2019benchmarking, wu2019behavior}, policy evaluation is a difficult problem in offline reinforcement learning, since the learned value functions, such as Q-values are often not a good indicator of the performance and if we cannot evaluate the policy properly, then we cannot improve the policy. Hence, to evaluate the learned policy from the data generated by the behavioral policy,  we have to leverage off-policy policy evaluation, as we shall introduce in the following.
 In order to address this distributional mismatch, many approaches have been proposed, we mainly categorize these methods into three parts: \textbf{model-based}, \textbf{model-free}, and \textbf{hybrid} ones, which are present in the following. Here, we merely give a bird's eye view of existing off-policy evaluation techniques and detailed discussions are included in the last subsection, where we look into the difference between them and those causality-based OPPE approaches. 

\subsection{Model-based} This type of methods circumvent this mismatch by first learning a MDP model from the observations (sample trajectories) and then use the learned model to evaluate the target policy. Specifically, model-based methods focus on constructing an approximation of the reward function $r(s,a)$ and/or the transition kernel $\Tfun(s,a,s')$. For example, both approximate models in \cite{jiang2016doubly, thomas2016data} rely on a reward function estimate of the underlying MDP model. For model estimation, the simplest method is probably the count-based estimation for discrete MDPs, where the reward function and the transition kernel are approximated based on observed state-action-reward tuples, leading to consistent maximum-likelihood estimators of the model. However, this method has no or limited generalization \cite{paduraru2013off}. If no samples are available for some state-action pair, then the associated estimation is not defined. Equipped with generalization, another common approach is regression estimator \cite{paduraru2013off, mannor2007bias} for continuous cases, which is essentially a representation learning for the MDP and its performance heavily depends on the selection of representation class and the design of loss functions. Moreover, we shall compare model-based estimators with causality-based model learning at the end of this section, where we show the advantage of counterfactual thinking during the model learning process.  
\subsection{Model-free}: Model-free methods are those which do not rely on the underlying MDP model. Most model-free methods \cite{guo2017using, precup2000eligibility, thomas2015high} aims directly at the distributional mismatch by importance sampling \cite{kahn1953methods}. As a technique in computational statistics, Importance Sampling (IS) computes an expected value under some distribution of interest by weighting the samples generated from some other distribution, which exactly fits the OPPE formulation. As introduced above, a sample trajectory $\tau=\left(s_{0}, a_{0}, \dots, s_{H}\right)$ with a distribution $p_{M,\mu}$, the empirical return $\sum_{t=0}^{H-1}r_t$ gives an unbiased estimate of the expected return $\mathbb{E}_{\tau\sim p_{M,\mu}}\{\sum_{i=0}^H r(s_t,a_t)\}$. If we define the per-step importance ratio as $\rho_t:=\pi(s_t,a_t)/\mu(s_t,a_t)$ and the cumulative importance ration as $\rho_{0:t}:=\prod_{k=0}^t \rho_k$, then the basic (trajectory-wise) IS estimator, and an improved step-wise version are given as follows:    
$$V_{\mathrm{IS}}:=\rho_{1: H} \cdot\left(\sum_{t=1}^{H} \gamma^{t-1} r_{t}\right),V_{\mathrm{step}-\mathrm{IS}}:=\sum_{t=1}^{H} \gamma^{t-1} \rho_{1: t} r_{t},$$ which is based on the fact that $p_{M,\pi}=d_{0}\left(s_{0}\right) \prod_{t=0}^{H-1}\left[\Tfun(s_t,a_t,s_{t+1}) \mu\left(s_{t}, a_{t}\right) \rho_t\right]$. For more details and variants such as weighted importance sampling, we refer readers to \cite{precup2000eligibility, thomas2015high}. 

Model-free methods provide one obvious advantage: they provide a consistent estimator with low bias, whereas model-based ones often suffer from higher bias, if the estimated model is a poor approximation. However, IS-based approach is far from perfect and there are two major issues with it: 1) typically, this approach tends to have high variance, especially when the target policy is deterministic. 2) It requires absolute continuity assumption regarding the polices. That is, for all state-action pairs $(s,a)\in \sset\times\aset$, if $\mu(s,a)=0$ then $\pi(s,a)=0$. This assumption requires that all state-action pairs $(s,a)$ produce by the target policy must have been observed in the sample trajectories, otherwise the importance ration $\rho_t$ cannot be defined. To sum up, there is no generalization in IS approach, meaning that we are unable to deal with the data we haven't seen before and in the following we shall see how causality-based model-free methods tackle these issues with counterfactual inference, enabling generalization in off-policy evaluation when facing unobserved data.   
\subsection{Hybrid}: There has been a growing interest in combining the two approaches for constructing unbiased estimators with low variances. The first attempt in this direction can be dated back to \cite{dudik2011doubly}, where a hybrid estimator named \textit{doubly robust} (DR) estimator, combining both model estimate and importance sampling, is proposed for policy evaluation in contextual bandits. This DR estimator admits the following form: $V_{\text{DR}}:=\widehat{V}(s)+\rho(r-\hat{r}(s,a)),$ where $\hat{r}$ is a good estimate of the reward function, $\widehat{V}$ is the expected reward under the policy $\pi$, defined as $\widehat{V}(s):=\mathbb{E}_{\pi}\{\hat{r}(s,a)\}$ and $\rho$ is the importance ratio. Simply put, we can treat this doubly robust estimator DR = model estimate + importance sampling. This idea is further developed in \cite{jiang2016doubly} and authors extend the DR for contextual bandit to a DR estimator for sequential decision-making.  By decomposing the whole trajectory into state-action-reward tuples, off-policy evaluation in reinforcement learning can be viewed as estimation in multiple contextual bandits problems, where $s_t$ is the state, $a_t$ is the action, and the observed return is defined recursively for adding the temporal relations in MDP to the rewards in the contextual bandit setting. Built upon this DR estimator, many variants have been proposed recently. In \cite{farajtabar2018more}, for the model-based part, a loss function (a weighted mean square error) is proposed for reducing the variance, yielding a better model estimation, which minimize the variance of the DR estimator. On the other hand, a novel approach for blending model-based and model-free parts is considered in \cite{thomas2016data}. In this work, model-based and model-free estimators are not applied to the sample trajectory at the same time, instead, authors first partition the whole trajectory into to parts, where the first half is handled by importance sampling and the rest by a model-based estimator. Naturally, different partitions lead to different estimates, blending model-free and model-based estimates together differently and the new estimator in this paper returns a weighted average of these blending estimates so as to minimize the mean square error.           
\section{Causality-based Off-Policy Policy Evaluation}
The idea behind causality-based off-policy policy evaluation is that the target policy is treated as a kind of intervention, comprising counterfactual actions that are different from the those in behavioral policy. Therefore, in order to evaluate the target policy based on observational data generated by the behavioral policy, we have to focus on the difference between the two policies or more specifically, the counterfactual outcomes. That is, \textit{what would have happened, had we applied those actions from the target policy}. In other words, with this counterfactual thinking, OPPE problem reduces to counterfactual inference problem and in this subsection, we shall present two approaches of leveraging causal inference in solving OPPE problem.   
\subsubsection{Model-free Approach: Counterfactually-guided Policy Evaluation}
The first approach does not rely on the underlying \textbf{MDP models}, and on the contrary, it casts MDPs into structrual causal models (SCM) for counterfactual inference, where actions in the target policy are viewed as interventions. We first introduce the generic approach of counterfactual inference then we move to its applications in OPPE, as studied in \cite{buesing2018woulda, oberst2019counterfactual}. 


On the other hand, as we discussed before, OPPE is also about answering a counterfactual question \textit{what would have happened, had we applied those actions from the target policy}. Hence, if we can represent any given MDP models or more broadly POMDP models by an SCM over trajectories \cite{buesing2018woulda}, and we treat those trajectories generated by the behavioral policy as observations, actions from the target policy as interventions, then we are also able to identify the expected return under the target policy using counterfactual inference, where the value function becomes the query variable. This one-to-one correspondence between counterfactual inference and OPPE, as shown in the Table\ref{cfi_oppe}, is built upon structural models that capture the underlying cause-effect relationship between variables, which has been the foundation for some research works on causality-based decision-making, such as multi-armed bandits problem \cite{bareinboimbandits15, zhang2017transfer} and reinforcement learning \cite{buesing2018woulda, oberst2019counterfactual}. In the sequel, we detail the SCM for addressing OPPE and explicitly express evaluation of the target policy as an intervention.
\begin{table}
\centering
	\begin{tabular}{ll}
	\toprule
	CFI& OPPE\\
	\midrule
	observations & off-policy episodes\\
	interventions  & target policy\\
	query variable  & expected return \\
	\bottomrule
\end{tabular}
\caption{Correspondence between Counterfactual Inference (CFI) and Off-Policy Policy Evaluation (OPPE)}
\label{cfi_oppe}
\end{table} 

In MDP (POMDP) or bandits problems, the casual relationships among variables are straightforward and we only need to care about those unobserved confounders when constructing SCMs. For example, in POMDP, the agent make a decision based on the history he has observed, which consists of the observation at each time step and the observation is determined by the state the agent is currently in. Meanwhile, the decision taken at this time step will lead the agent to the next state, which in turn influence future's observations. The DAG for this POMDP example is provided in Fig\ref{dag_pomdp}, where the unobserved confounders in POMDP are also included. According to the DAG, in the SCM, we can express the transition kernel $\Tfun(\st{t},\at{t},\st{t+1})$ as deterministic functions with independent noise variables $U$, such as $\st{t+1}=f_{st}(\st{t},\at{t},U_{st})$, which is always possible using auto-regressive uniformization \cite{buesing2018woulda}. Accordingly, we express a given policy $\pi$ as a causal mechanism: $\at{t}=f_\pi(H_t,U_{at})$, therefore, Running the target policy $\pi$ instead of the behavioral policy $\mu$ in the environment can be viewed as an intervention $I(\mu\rightarrow \pi)$ consisting of replacing $\at{t}=f_\mu(H_t,U_{at})$ by $\at{t}=f_\pi(H_t,U_{at}).$     
\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{dag_pomdp}
	\caption{DAG for the POMDP example, taken from \cite{buesing2018woulda}: $\st{t}$ denotes the state at time $t$. $H_t:=(O_1,A_1, O_2,A_2, \cdots, A_{t-1}, O_{t})$ is the set of historical observations up to time $t$. $U_{o_t}, U_{s_t}$ denote the unobserved confounders for the observation $O_t$ and $\st{t}$ respectively.}
	\label{dag_pomdp}
\end{figure}    

\subsubsection{Model-based: Counterfactually-guided Model Learning}
Different from model-free methods that completely bypass MDP models, model-based ones still rely on the underlying MDP model learned from the observational data generated from the behavioral policy for evaluating the target policy. One of the key challenges in model leaning is the choice of the loss function for model learning without the knowledge of the evaluation policy (or the distribution of the evaluation policies). Without this knowledge, we may select a loss function that focuses on learning the areas that are irrelevant for the evaluation policy. Different from previous model-based methods which only take into account data generated by behavioral policy, a new loss function is proposed involving counterfactual thinking when learning the representation using neural networks \cite{liu2018representation}, which bakes target policy evaluation into representation learning process. This make the learned model more suitable for OPPE, compared with models only involves behavioral data.    

To be more specific, for an unknown MDP model $M=\langle r(s,a), \Tfun({s,a,s'})\rangle$, we can learn a model $\widehat{M}=\left\langle\widehat{r}(s, a), \widehat{\Tfun}\left(s, a, s'\right)\right\rangle=\left\langle h_{r}(\phi(s), a), h_{\Tfun}\left(\phi(s\right), a,\phi(s^{\prime})\right\rangle$, which is based on the representation function $\phi$, i.e., neural networks. Here, $\phi: \sset\rightarrow \mathcal{Z}$ is a reversible and twice-differentiable function, where $\mathcal{Z}$ is the representation space. The procedure of model-based approach comprises two steps: we first learn the representation $\phi$ based on the historical data and a carefully selected loss function, derived from counterfactual thinking. Then, we evaluate the target policy using the learned model $\widehat{M}$, which is the same as the classical model-based methods. In this subsection, we mainly focus on the first step, presenting how counterfactual thinking leads to a suitable representation for evaluating the target policy in model learning. Before we move to the details, we first introduce the following notations.  For $\tau=\left(s_{0}, a_{0}, \dots, s_{H}\right)$, a trajectory of $H + 1$ states and actions from model $M$, generated by the policy $\mu$, we define the joint distribution of $\tau$ as $p_{M,\mu}=d_{0}\left(s_{0}\right) \prod_{t=0}^{H-1}\left[\Tfun(s_t,a_t,s_{t+1}) \mu\left(s_{t}, a_{t}\right)\right]$, where $d_0$, as introduced at the beginning of this section, is the initial state distribution. Accordingly, we can define the associated marginal and conditional distributions as $p_{M, \mu}\left(s_{0}\right), p_{M, \mu}\left(s_{0}, a_{0}\right)$. With these distributions, we can define the $t-$step value function of policy $\mu$ as $V_{M,t}^\mu(s)=\mathbb{E}_{\tau\sim p_{M,\mu}(s_0)}\{\sum_{i=0}^t a_i\}$. Similarly, for the estimated model $\widehat{M}$ and the target policy $\pi$, we can define distributions and value functions in the same way. 


Now we are in a position for illustrating the combination of counterfactual thinking and mode-based OPPE that leads to a more data-efficient framework for evaluating the target policy, which is first introduced in \cite{liu2018representation}. Specifically, the key of this framework is that this combination provides a loss function that takes target policy into consideration by counterfactual inference, resulting in a learned model that is suitable for evaluating the tagret policy. Theoretically, for the behavioral policy $\mu$ and the target policy $\pi$, the actual difference is measured by $\mathbb{E}_{s_0\sim \isset}\left(V_{M}^{\pi}\left(s_{0}\right)-V_{M}^{\mu}\left(s_{0}\right)\right)^2$. However, we do not know the underlying MDP model $M$ and can only estimate it based on history data, which we shall detail in the sequel. For now, we assume a learned model $\widehat{M}$ is available, then OPPE relies on the estimated difference$(V^{\pi}_{\widehat{M}}\left(s_{0}\right)-V^{\mu}_{\widehat{M}}\left(s_{0}\right))$. One natural question is how different are the actual difference $\left(V_{M}^{\pi}\left(s_{0}\right)-V_{M}^{\mu}\left(s_{0}\right)\right)$ and the estimated one $(V^{\pi}_{\widehat{M}}\left(s_{0}\right)-V^{\mu}_{\widehat{M}}\left(s_{0}\right))$? To answer this question, we first look at the following upper-bound, which is straightforward by using Cauchy-Schwartz inequality. $$\frac{1}{2} \mathbb{E}_{s_{0}\sim\isset}\left[(V_{\widehat{M}}^{\pi}(s_{0})-V_{\widehat{M}}^{\mu}\left(s_{0})\right)-(V_{M}^{\pi}(s_{0})-V_{M}^{\mu}(s_{0}))\right]^{2} \leq \mathrm{MSE}_{\pi}+\mathrm{MSE}_{\mu},$$
  where $\text{MSE}_\pi:=\mathbb{E}_{s_{0}\sim \isset}\left(V_{\widehat{M}}^{\pi}\left(s_{0}\right)-V_{M}^{\pi}\left(s_{0}\right)\right)^{2}$ and $\text{MSE}_\mu:=\mathbb{E}_{s_{0}\sim\isset}\left(V_{\widehat{M}}^{\mu}\left(s_{0}\right)-V_{M}^{\mu}\left(s_{0}\right)\right)^{2}$ are the mean-squared error for two policy value estimates. The above inequality tells that the difference is upper-bounded by the sum of two MSEs, and once we can find a representation $\phi$ such that this upper-bound $\text{MSE}_\pi+\text{MSE}_\mu$ is minimized with respect to the representation, then the estimated difference serves as a fairly good evaluation of the target policy. Therefore, the problem reduces to express the upper-bound as a functional of $\phi$, since $\widehat{M}$ is merely a notation and it is the reward function $\hat{r}(s,a)=h_{r}(\phi(s), a)$and the transition kernel $\hat{P}=h_{\Tfun}\left(\phi(s\right), a,\phi(s^{\prime})$ that explicitly depend on the $\phi$. This is where counterfactual inference plays a part, as we shall see in the following.
  
  For $\text{MSE}_\mu=\mathbb{E}_{s_{0}\sim\isset}\left(V_{\widehat{M}}^{\mu}\left(s_{0}\right)-V_{M}^{\mu}\left(s_{0}\right)\right)^{2}$, we know the behavioral policy and have the sampled trajectories, hence for this on-policy case, we can apply the Simulation Lemma \cite{kearns2002near}, showing that this on-policy mean square error cane be upper bounded by a function of the reward and transition prediction losses. This upper-bound is provided in the following inequality.
 \begin{align*}
 	\mathbb{E}_{s_{0}}\left[V_{\widehat{M}}^{\mu}\left(s_{0}\right)-V_{M}^{\mu}\left(s_{0}\right)\right]^{2} \leq 2 H \sum_{t=0}^{H-1} \mathbb{E}_{s_{t}, a_{t} \sim p_{M, \mu}}\left[\bar{\ell}_{r}\left(s_{t}, a_{t}, \widehat{M}\right)+\bar{\ell}_{T}\left(s_{t}, a_{t}, \widehat{M}\right)\right],
 \end{align*}          
 where $\bar{\ell}_{r}\left(s_{t}, a_{t}, \widehat{M}\right)$ and $\bar{\ell}_{T}\left(s_{t}, a_{t}, \widehat{M}\right)$ are the prediction losses of the reward function and the transition kernel respectively and are defined as follows
 \begin{align*}
 	&\bar{\ell}_{r}\left(s_{t}, a_{t}, \widehat{M}\right):=\left(\widehat{r}\left(s_{t}, a_{t}\right)-r\left(s_{t}, a_{t}\right)\right)^{2}, \\
 	&\bar{\ell}_{T}\left(s_{t}, a_{t}, \widehat{M}\right):=\left(\int_{\mathcal{S}}\left(\widehat{\Tfun}\left( s_{t}, a_{t}, s^{\prime}\right)-\Tfun\left(s_{t}, a_{t}, s^{\prime}\right)\right) V_{\widehat{M}, H-t-1}^{\mu}\left(s^{\prime}\right) d s^{\prime}\right)^{2}.
 \end{align*}
 However, the difficulty here is that we do not have on-policy data for the target policy $\text{MSE}_\pi$ and this is why we need counterfactual thinking for constructing an upper bound for $\text{MSE}_\pi$. In \cite{liu2018representation}, authors decompose the value function error into a onestep reward loss, a transition loss and a next step value loss, with respect to the on-policy distribution. Then, this becomes a contextual bandit problem, and estimation of the MSE is equivalent to the estimation of treatment effect, where the intervention is replacing the behavioral policy $\mu$ with the target policy $\pi$. This approach is built upon Shalit et al.’s work \cite{shalit2017estimating} about binary action bandits, where the distribution mismatch is bounded by a representation distance penalty term.
\subsection{Analysis}   
If we dive deeper into these causal approaches, we can find that it is the generalization brought up by causal inference that helps solve OPPE problems. Intrinsically, dealing with off-policy evaluation is nothing else but making a prediction about the decision-making system under counterfactual interventions. From this perspective, we argue that causality enhance the generalization of previous off-policy evaluation methods by transferring the cause-effect relationship we infer from observations to the target policy evaluation process. In other words, we are able to handle the ``missing data'', i.e., the sate-action-reward tuples included in the target policy that are absent from the sample trajectories generated by the behavioral policy. Specifically, in this subsection, we compare causality-based approaches with existing off-policy evaluation techniques as we briefly introduced at the beginning of this section, showing that how causality equips these novel approaches with better generalization. 

Traditional model-free methods, as we have briefly reviewed above, are rather restrictive in the sense that they often need absolute continuity assumption for computing the importance ratio $\rho_t=\pi(s_t,a_t)/\mu(s_t,a_t)$ and besides this, as we can see from the definition of $\rho_t$, this ratio requires the explicit knowledge of the behavioral policy, i.e., the distribution regarding $\mu$. However, in practice, it so happens that we either do not know the behavioral policy $\mu$ or the sample trajectories are in fact generated by multiple behavioral policies. Moreover, absolute continuity is usually not satisfied in real-world applications, which is a major limit of its wider applications, since there is no generalization within this model-free framework. Even though, as mentioned in \cite{jiang2016doubly, farajtabar2018more}, when the importance ratio is not defined or the behavioral policy is unknown, they can be estimated from the data using some parametric function classes and a good example of estimating the behavioral policy is provided in \cite{farajtabar2018more}, we think that these remedies do not address the poor generalization of importance sampling directly, which heavily depends on the quality of observations, since they merely try to create the missing pieces of importance sampling.

Causality make it possible that estimators that do not rest on MDP models are still able to generalize well by incorporating SCMs. Though one may argue that this is not model-free anymore, as this approach involves SCMs, we believe that requiring causal models is the price we have to pay for bypassing the MDP models while acquiring generalization ability, which we shall illustrate later. We first clarify that the term ``model-free'' indicates that this causal approach circumvents complicated MDP models involving both reward and transition kernel estimation and turns to causal models, which are much easier to deal with, since causal relationships are straightforward in MDP setting, e.g., it is the last sate and action as well as unobserved confounders that lead to the current state. Now we are in a position to elaborate on the advantages of this causality-based model-free approach, as shown below.
\begin{itemize}
  \item \textbf{Generalization} As we have introduced above, this causal approach do not address the distribution mismatch by importance sampling, instead it first provides a SCM, based on which a counterfactual inference is conducted to evaluating the target policy. In other words, as long as the historical observations produce a good estimate of the unobserved confounders and causal mechanisms, we do not care whether absolute continuity is satisfied or not, since it is no longer the key of the estimation. This generalization from observed actions in sample trajectories to counterfactual actions from the target policy is essentially based on the estimated SCM . 
  \item \textbf{Unbiased Estimation} Another advantage of this causal approach is it gives unbiased estimates, if the trajectory distribution of the behavioral policy entailed by the SCM coincides with the actual one distribution entailed by the MDP. This shows that causality-based approach returns a consistent evaluation of the target policy, which is different from MDP model-based estimation.  
\end{itemize}
    However, a successful implementation of this model-free usually requires the following crucial assumptions. 1) There are no additional hidden confounders, otherwise the current SCM and CFI are invalid. 2) Causal Mechanisms such as transition kernel and reward functions are easy to model and 3) the inference over the noise $U$ given data to be sufficiently accurate. The first assumption is merely a technical one while the second one can be carefully handled by parametric function classes, e.g., neural nets. The last one plays a significant role, and as discussed in \cite{buesing2018woulda}, imperfect inference over the scenario $U$ could result in wrongly attributing a negative outcome to the agent’s actions, instead environment factors. Hence further investigation is needed for measuring the quality of inference.          

On the other hand, different from traditional model-free methods, most current model-based methods comprising model learning/estimation process inherently possess generalization to some extent, since the learned model parameters can be directly leveraged when dealing with a new policy without any alterations. However, as pointed out in \cite{farajtabar2018more}, there are two major problems with these model-based approaches: (1) Its bias cannot be easily quantified, since in general it is difficult to quantify the approximation error of a function class, and (2) It is not clear how to choose the loss function for model learning. The first problem is more about a choice of representations and causality cannot help with that but as we have shown in the last subsection, causal inference can bring a more reasonable loss function for model learning. Without causality, we are unable to acquire some prior knowledge about the target policy and generalize from observations and the common way for designing the loss function is to look at the empirical risk of evaluating the behavioral policy using the model estimation, which reduces the problem to the on-policy model learning. However, as discussed in \cite{liu2018representation}, this kind of model learning yields a model that is suitable for evaluating the behavioral policy instead of the target policy, since the representations are chosen in such a way that the estimation error of the behavioral policy is minimized. 

Causality make it possible that taking the target policy into account when designing the model learning. 



==> outline.tex <==
\section{Introduction}
\begin{enumerate}
    \item Two equivalent counterfactual questions
    \item important in overlapping domains (e.g: health) where new data is expensive and/or mistakes during online training are unacceptable.
    
\end{enumerate}
\hrule
\begin{itemize}
  \item Offline RL and off-policy evaluation
  \begin{itemize}
      \item Offline RL involves asking questions about missing data, specifically what whould have happened had I used policy $\hat{\pi}$ instead of $\pi$ which generated it.
      \[
      V^{\hat{\pi}}\geq V^\pi -\epsilon
      \]
      \item These are counter-factual questions, we care about improvement. 
      \item In causality, we have similar issues which are estimating what would have happened
      \[
      ATE=E\{Y|x=1\}-E\{Y|X=0\}
      \]
  \end{itemize}
  \item Connections with causal inference
\end{itemize}
\section{Causality}
\begin{itemize}
  \item Basics: DAG, SCM, and etc
  \item Average treatment effect, do-calculus 
  

\end{itemize}
\section{Causality-based Off-Policy Evaluation}
\begin{itemize}
  \item Generic approaches of leveraging causal inference
  \begin{itemize}
  \item Casting MDPs into SCMs for counterfactual inference (model free)
  \item Incorporating ATE into MDPs for better models (model based)
\end{itemize}
    \item Problems with traditional methods: model-based, model-free and hybrid ones
 	\item Advantages over traditional ones
\end{itemize}






\section{Our comments}
\begin{itemize}
  \item What makes causality so important in OPE
  \item What else causality can do in RL 
  \item What are the challenges (limitations) 
  \item Algorithmic issues: How do these two groups try to 
\end{itemize}
\newpage

==> scratch.tex <==

\subsection{Best practices for exploring data}
\subsubsection{Exploring the domain space in in RL}
Hanna et al [1] explore the notion of a \textit{behavior policy}, a policy for exploring the RL problem domain which will minimize the offline estimates for batch reinforcement learning. They define an equation 

\includegraphics[scale=1]{is_behavior.png}

where $IS(H, \theta)$ is the weighted importance sampling return of a trajectory, $H$, sampled from a behavior policy, $\pi_\theta$ with parameters $\theta$, minimizing the mean squared error in the reward estimate. The authors propose an update algorithm based on the above gradient to continually refine the behavior policy so as to reduce the error estimate. The method of exploration, $\pi_\theta$, is thus updated after every sampling.

\subsubsection{Exploring the domain space in in Causality}

Under the view of causality, this problem be seen as an effort to discover the right causal graph so as to minimize the error in a proposed treatment effect. Pearl discusses the IC (Inductive Causation) and IC* (Inductive Causation with latent variables) as ways to uncover a causal graph given a fixed distribution $P$, algorithms which largely consist of adding single edges to unconnected variables in the causal structure and testing for consistency with observed data. 
While the inductive causation algorithms don't include a way to  update the experiments producing the distribution $P$, several other methods discuss this. 

* https://arxiv.org/pdf/1809.09337.pdf
* https://www.frontiersin.org/articles/10.3389/fgene.2019.00524/full

\subsection{Estimating errors}

Hana et al [1] similarly discuss how in reinforcement learning, the expected between the reward of an actual policy and the actual reward of an effect can be seen through a doubly robust estimator.

In causality, we can similarly discuss the average treatment effect of a variable $x$ being turned on or off as 

$$\tau(x) = \mathbb{E}[y|x, t=1] -\mathbb{E}[y|x, t=0]$$

where $\tau(x)$ is the cumulative average treatment effect, $y$ is the outcome, and $t=1$ represents the treatment being turned on for variable $x$. 

The mean squared error of the value of all such $y$'s then leads to a cumulative average treatment effect called the \textit{precision in estimation of heterogeneous effect} (PEHE).

$$\epsilon_{PEHE} = \frac{1}{n} \sum_{i=1}^{n}(y_i^{1} - y_i^{0} - \tau(x_i))^2$$

This notion of error is different from the doubly robust estimators in that it seeks to understand the cumulative error from all variables rather than the error for a given policy.

https://arxiv.org/pdf/0804.2958.pdf 
https://arxiv.org/pdf/2002.02836.pdf
[1] https://arxiv.org/pdf/1706.03469.pdf
[2] https://arxiv.org/pdf/1809.09337.pdf
[3]https://imai.fas.harvard.edu/research/files/Design.pdf
[4]https://arxiv.org/pdf/1702.08567.pdf

\subsection{Theoretical limits on the lower bound}

\subsection{Data format}

* meta reinforcement learning, discovering causal relationships
* automated causality discovery
https://arxiv.org/pdf/1702.08567.pdf
https://arxiv.org/pdf/1809.09337.pdf
https://imai.fas.harvard.edu/research/files/Design.pdf
https://www.frontiersin.org/articles/10.3389/fgene.2019.00524/full
